AdaCache: A Disaggregated Cache System with Adaptive Block Size for Cloud Block Storage

NVMe SSD caching has demonstrated impressive capabilities in solving cloud block storage's I/O bottleneck and enhancing application performance in public, private, and hybrid cloud environments. However, traditional host-side caching solutions have several serious limitations. First, the cache cannot be shared across hosts, leading to low cache utilization. Second, the commonly-used fix-sized cache block allocation mechanism is unable to provide good cache performance with low memory overhead for diverse cloud workloads with vastly different I/O patterns. This paper presents AdaCache, a novel userspace disaggregated cache system that utilizes adaptive cache block allocation for cloud block storage. First, AdaCache proposes an innovative adaptive cache block allocation scheme that allocates cache blocks based on the request size to achieve both good cache performance and low memory overhead. Second, AdaCache proposes a group-based cache organization that stores cache blocks into groups to solve the fragmentation problem brought by variable-sized cache blocks. Third, AdaCache designs a two-level cache replacement policy that replaces cache blocks in both single blocks and groups to improve the hit ratio. Experimental results with real-world traces show that AdaCache can substantially improve I/O performance and reduce storage access caused by cache miss with a much lower memory usage compared to traditional fix-sized cache systems.

==> acknowledgement.tex <==
\Section{Acknowledgements}
\label{sec:acknowledgement}
This work was supported by Samsung Semiconductor. 

==> alibaba_replay_wss10.tex <==
rd_avg_lat_us	2.csv	10.csv	49.csv	124.csv	740.csv
var	368.02	226.924	412.71	136.62	68
32k	451.306	329.335	484.742	142.35	84
64k	371.652	228.644	416.925	140.727	94
128k	489.29	251.596	503.885	167.968	177
256k	934.763	385.172	730.19	223.774	186
					
wr_avg_lat_us	2.csv	10.csv	49.csv	124.csv	740.csv
var	110.558	98.4213	315.94	114.247	222.437
32k	141.215	122.101	392.075	184.425	307.25
64k	118.607	107.671	319.961	116.331	235.751
128k	134	110.639	373.944	124.075	245.751
256k	214.304	136.78	562.435	228.751	378.878


process_each_req_lat_us	2.csv	7.csv	10.csv	21.csv	49.csv	124.csv	207.csv	740.csv	804.csv	810.csv
32k	3.09	1.48	3.64	2.37	6.40	8.57	35.97	5.04	25.34	37.38
64k	2.77	1.32	2.94	1.86	5.50	6.19	20.84	4.24	15.80	23.86
128k	2.41	1.25	2.34	1.49	4.33	4.45	16.13	3.14	9.78	13.96
256k	2.16	1.14	1.90	1.31	3.69	2.70	9.56	2.53	7.46	10.25
32k-256k	2.74	1.40	2.81	2.17	5.06	8.44	29.76	4.18	18.56	27.91

32k-256k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
2.00	3059595.00	71358614016.00	9748224.00	146804946944.00	1051716.00	59268300800.00	903252.00	39598686208.00	903252.00	39598686208.00	2096975.00	1543611.00	7903024.00	7410502.00	29705.00
7.00	212957.00	4526166016.00	10427955.00	86336531968.00	198077.00	11718787072.00	64174.00	3302195200.00	64174.00	3302195200.00	249414.00	110572.00	9750585.00	9692943.00	105216.00
124.00	12539986.00	259059277824.00	3961438.00	181538869248.00	3223552.00	174136557568.00	178448.00	7437254656.00	178448.00	7437254656.00	9287708.00	6352898.00	712291.00	589944.00	494007.00
10.00	8982348.00	97785897472.00	2008113.00	68650299904.00	305614.00	51317768192.00	540646.00	38060883968.00	540646.00	38060883968.00	8315112.00	8120671.00	1684887.00	1575337.00	551938.00
49.00	8860297.00	237916126208.00	7258018.00	200215878144.00	2650101.00	158219468800.00	2210354.00	97889419264.00	2210354.00	97889419264.00	4824277.00	3509318.00	5175722.00	3888760.00	564097.00
21.00	1046977.00	34394890240.00	12033346.00	195410329600.00	1046737.00	34472263680.00	1046907.00	34394079232.00	1046907.00	34394079232.00	120.00	5.00	9999879.00	8953436.00	566271.00
207.00	13180348.00	614459826176.00	15317131.00	1728027331072.00	3113597.00	1052814376960.00	4421479.00	269097074688.00	4421479.00	269097074688.00	5566824.00	3532411.00	4433175.00	3372142.00	6552424.00
740.00	2679522.00	109499973632.00	11165192.00	183710474240.00	2374736.00	115393200128.00	2679522.00	109499973632.00	2679522.00	109499973632.00	1.00	0.00	9999998.00	7782132.00	6689428.00
804.00	19105103.00	1036546576384.00	3382305.00	659520364544.00	1761061.00	592597647360.00	6056438.00	431518089216.00	6056438.00	431518089216.00	8383294.00	7946814.00	1616705.00	298948.00	8158766.00
810.00	15387888.00	726018408448.00	9500142.00	1206154436608.00	6419665.00	1126560104448.00	6411450.00	426578935808.00	6411450.00	426578935808.00	7006988.00	2084357.00	2993011.00	1520861.00	9743363.00
															
32k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
2.00	3599382.00	72340612096.00	10030390.00	148022891008.00	1083318.00	61047570432.00	1242586.00	40717058048.00	1242586.00	40717058048.00	2096975.00	1525167.00	7903024.00	7394270.00	36281.00
7.00	239769.00	4272377856.00	10367570.00	86439284224.00	198051.00	11637620736.00	94053.00	3081928704.00	94053.00	3081928704.00	249414.00	108112.00	9750585.00	9693952.00	130850.00
124.00	13294164.00	248809160704.00	4144741.00	197454929920.00	3391177.00	190140416000.00	234208.00	7674527744.00	234208.00	7674527744.00	9287708.00	6118652.00	712291.00	588435.00	577310.00
10.00	9594501.00	97716096512.00	2095169.00	72767103488.00	431311.00	55479894016.00	1174205.00	38476349440.00	1174205.00	38476349440.00	8315112.00	7993675.00	1684887.00	1575140.00	680596.00
49.00	10688259.00	242531648000.00	7415596.00	203664304640.00	2710138.00	162516008960.00	3149643.00	103207501824.00	3149643.00	103207501824.00	4824277.00	3499833.00	5175722.00	3816616.00	695498.00
21.00	1238372.00	40577490944.00	11633598.00	200173080576.00	1232562.00	40647917568.00	1238302.00	40576679936.00	1238302.00	40576679936.00	120.00	5.00	9999879.00	8767438.00	697519.00
207.00	14364449.00	617488261120.00	9674332.00	1727689422848.00	3100128.00	1052828958720.00	8284231.00	271457681408.00	8284231.00	271457681408.00	5566824.00	3531016.00	4433175.00	3369786.00	11664730.00
740.00	3662152.00	120001396736.00	11264960.00	189264900096.00	2606634.00	125887545344.00	3662152.00	120001396736.00	3662152.00	120001396736.00	1.00	0.00	9999998.00	7582508.00	11844360.00
804.00	24747815.00	1047575056384.00	3109475.00	649502924800.00	1668230.00	583142899712.00	13187710.00	432134881280.00	13187710.00	432134881280.00	8383294.00	8033864.00	1616705.00	298284.00	15068724.00
810.00	24079293.00	713438502912.00	10285427.00	1220223090688.00	6458429.00	1141908537344.00	13012043.00	426378625024.00	13012043.00	426378625024.00	7006988.00	2022546.00	2993011.00	1519097.00	18347988.00
															
64k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
2.00	2818180.00	86029558272.00	9219530.00	173493551616.00	971199.00	84822196224.00	814655.00	53389230080.00	814655.00	53389230080.00	2096975.00	1574742.00	7903024.00	7454427.00	18140.00
7.00	229226.00	5326884864.00	10125830.00	88228105728.00	136105.00	13382516736.00	53621.00	3514105856.00	53621.00	3514105856.00	249414.00	149151.00	9750585.00	9714783.00	65424.00
124.00	10672469.00	266754281472.00	3486961.00	243034689536.00	2759590.00	235073830912.00	130398.00	8545763328.00	130398.00	8545763328.00	9287708.00	6627400.00	712291.00	639713.00	288653.00
10.00	8993543.00	98755849216.00	1937121.00	73901777408.00	265732.00	55364026368.00	589022.00	38602145792.00	589022.00	38602145792.00	8315112.00	8149859.00	1684887.00	1584434.00	340295.00
49.00	7800458.00	284961175552.00	6963696.00	275508341760.00	2563276.00	233121906688.00	2229369.00	146103926784.00	2229369.00	146103926784.00	4824277.00	3523994.00	5175722.00	3918283.00	347745.00
21.00	635318.00	41632092160.00	10928277.00	205636644864.00	633669.00	41701277696.00	635223.00	41629974528.00	635223.00	41629974528.00	120.00	47.00	9999879.00	9366283.00	348755.00
207.00	10186907.00	642941710336.00	9176767.00	1745866444800.00	2866401.00	1058064433152.00	4163167.00	272837312512.00	4163167.00	272837312512.00	5566824.00	3724149.00	4433175.00	3409856.00	5832360.00
740.00	2150625.00	140943360000.00	10764246.00	222353608704.00	1778644.00	146829475840.00	2150625.00	140943360000.00	2150625.00	140943360000.00	1.00	0.00	9999998.00	8282213.00	5922174.00
804.00	17350084.00	1047311855616.00	3107037.00	667261476864.00	1605367.00	583736229888.00	6595628.00	432251076608.00	6595628.00	432251076608.00	8383294.00	8031936.00	1616705.00	362903.00	7534355.00
810.00	15765066.00	756740526080.00	9567095.00	1238269755392.00	6212437.00	1142179233792.00	6508484.00	426540007424.00	6508484.00	426540007424.00	7006988.00	2127808.00	2993011.00	1659785.00	9173986.00
															
128k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
2.00	2383408.00	109095709184.00	8825534.00	224420600320.00	895321.00	132665049088.00	579277.00	75926994944.00	579277.00	75926994944.00	2096975.00	1590759.00	7903024.00	7514007.00	9069.00
7.00	229446.00	6700589056.00	9983155.00	90818887680.00	93703.00	15960375296.00	32620.00	4275568640.00	32620.00	4275568640.00	249414.00	180651.00	9750585.00	9725658.00	32710.00
124.00	9492619.00	297925292032.00	2731468.00	302156730368.00	2016479.00	293677957120.00	74165.00	9720954880.00	74165.00	9720954880.00	9287708.00	7317751.00	712291.00	669217.00	144324.00
10.00	8668215.00	99755851776.00	1851358.00	76853965312.00	182457.00	55982686208.00	296945.00	38921175040.00	296945.00	38921175040.00	8315112.00	8223693.00	1684887.00	1593856.00	170144.00
49.00	6281299.00	363749493248.00	6681551.00	417426019328.00	2396451.00	372738490368.00	1715681.00	224877740032.00	1715681.00	224877740032.00	4824277.00	3579350.00	5175722.00	4025200.00	173868.00
21.00	327182.00	42873544704.00	10436594.00	209142321152.00	326590.00	42941808640.00	327075.00	42870374400.00	327075.00	42870374400.00	120.00	80.00	9999879.00	9673329.00	174372.00
207.00	8000024.00	687518744576.00	8625616.00	1780747423744.00	2658823.00	1066960027648.00	2097655.00	274943836160.00	2097655.00	274943836160.00	5566824.00	3886057.00	4433175.00	3455245.00	2916174.00
740.00	1256554.00	164699045888.00	10418247.00	256881827840.00	1135432.00	170585096192.00	1256554.00	164699045888.00	1256554.00	164699045888.00	1.00	0.00	9999998.00	8876747.00	2961080.00
804.00	12820221.00	1046892957696.00	2961177.00	701026070528.00	1493119.00	584784936960.00	3299633.00	432489496576.00	3299633.00	432489496576.00	8383294.00	8027353.00	1616705.00	479611.00	3767170.00
810.00	11226641.00	840086155264.00	8922147.00	1272134852608.00	5907998.00	1142908911616.00	3256322.00	426812637184.00	3256322.00	426812637184.00	7006988.00	2292128.00	2993011.00	1799880.00	4586985.00
															
256k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
2.00	2131732.00	155018174464.00	8647682.00	335257202176.00	874484.00	238823145472.00	465104.00	121924222976.00	465104.00	121924222976.00	2096975.00	1565696.00	7903024.00	7559824.00	4534.00
7.00	231897.00	8428503040.00	9885616.00	94899517440.00	66198.00	19888340992.00	20844.00	5464129536.00	20844.00	5464129536.00	249414.00	202042.00	9750585.00	9731762.00	16354.00
124.00	8979406.00	327905325056.00	2127415.00	393640833024.00	1417807.00	384598016000.00	43316.00	11355029504.00	43316.00	11355029504.00	9287708.00	7896332.00	712291.00	685903.00	72160.00
10.00	8490057.00	100755016704.00	1805792.00	79543288320.00	137279.00	56928239616.00	149449.00	39177158656.00	149449.00	39177158656.00	8315112.00	8261716.00	1684887.00	1601004.00	85069.00
49.00	5521289.00	507395414528.00	6501904.00	682855096320.00	2241703.00	634206027776.00	1398657.00	366649540608.00	1398657.00	366649540608.00	4824277.00	3643535.00	5175722.00	4114801.00	86930.00
21.00	171352.00	44894285824.00	10166262.00	212310261760.00	171114.00	44962676736.00	171244.00	44890587136.00	171244.00	44890587136.00	120.00	97.00	9999879.00	9828788.00	87181.00
207.00	6795473.00	773516918784.00	7975260.00	1848764648448.00	2434223.00	1082309476352.00	1060157.00	277913796608.00	1060157.00	277913796608.00	5566824.00	4037530.00	4433175.00	3528250.00	1458081.00
740.00	762743.00	199948500992.00	10218459.00	300111351808.00	739090.00	205834420224.00	762743.00	199948500992.00	762743.00	199948500992.00	1.00	0.00	9999998.00	9260910.00	1480533.00
804.00	10762194.00	1068943962112.00	2676400.00	719818420224.00	1251883.00	586971611136.00	1651629.00	432964632576.00	1651629.00	432964632576.00	8383294.00	8198221.00	1616705.00	549895.00	1883577.00
810.00	8944204.00	1050480783360.00	6315386.00	1308474368000.00	3454612.00	1143936647168.00	1630066.00	427312021504.00	1630066.00	427312021504.00	7006988.00	4646671.00	2993011.00	1898716.00	2293484.00
															


==> data.tex <==
Alibaba-0.05	read_hit_%		Alibaba-0.05	write_volume_TB
32k	64.14		32k	288
64k	66.98		64k	292
128k	68.90		128k	300
256k	70.19		256k	314.0518196
512k	69.81		512k	341.7173615
variable-32-128	64.52		variable-32-128	289
variable-32-256	64.59		variable-32-256	289
variable-32-512	64.80		variable-32-512	288
				
Alibaba-0.05	read_all_volume_TB		Alibaba-0.05	total_blocks
32k	131.62		32k	49412622.00
64k	176.45		64k	24706561.00
128k	263.07		128k	12353539.00
256k	432.81		256k	6177026.00
512k	730.51		512k	3088771.00
variable-32-128	130.94		variable-32-128	22240825.00
variable-32-256	130.90		variable-32-256	19684150.00
variable-32-512	130.58		variable-32-512	19530266.00

msr-0.05	read_hit_%		msr-0.05	write_volume_TB
32k	88.36		32k	1.49
64k	88.20		64k	1.90
128k	89.86		128k	2.95
256k	91.08		256k	5.17
512k	88.28		512k	9.07
variable-32-128	86.54		variable-32-128	1.71
variable-32-256	86.37		variable-32-256	1.81
variable-32-512	88.28		variable-32-512	1.68
				
msr-0.05	read_all_volume_TB		msr-0.05	total_blocks
32k	9.51		32k	4807249.00
64k	12.29		64k	2403635.00
128k	13.81		128k	1201824.00
256k	16.29		256k	600921.00
512k	17.17		512k	300472.00
variable-32-128	9.59		variable-32-128	2968343.00
variable-32-256	9.60		variable-32-256	2919007.00
variable-32-512	8.64		variable-32-512	2932614.00


msr-0.05	read_hit_%		msr-0.05	write_volume_TB
32k	77.05		32k	14.24
64k	81.52		64k	16.05
128k	85.02		128k	19.52
256k	87.50		256k	26.41
512k	85.90		512k	38.54
variable-32-128	76.56		variable-32-128	14.93
variable-32-256	76.42		variable-32-256	15.10
variable-32-512	76.34		variable-32-512	15.16
				
msr-0.05	read_all_volume_TB		msr-0.05	total_blocks
32k	102.43		32k	12941953.00
64k	122.45		64k	6470979.00
128k	151.90		128k	3235491.00
256k	195.09		256k	1617746.00
512k	217.99		512k	808874.00
variable-32-128	103.10		variable-32-128	7940922.00
variable-32-256	103.49		variable-32-256	7821821.00
variable-32-512	103.77		variable-32-512	7878286.00

	read bandwidth	read bw stddev	read IOPS	read iops stddev	read Latency	read lat stddev	write bandwidth	write bw stddev	write IOPS	write iops stddev	write Latency	write lat stddev
local	4377	5.64	1121	1.44	173.18	99.97	4377	5.66	1121	1.44	48.98	19.6
nvmeof	4109	31.57	1016	8.08	172.35	80.78	4109	31.57	1016	8.08	75.91	23.01
rbd	74.4	1.62	18.2	0.4	3468	10504.3	70.9	1.61	18.1	0.4	10545	17836.37

read_volume_gb	read_io_cnt	write_volume_gb	write_volume_cnt
alibaba	607.35	24524073.00	375.97	25475922.00
msr	2416.84	60960448.00	207.23	9039545.00
systor	1109.21	40725672.00	271.91	19274322.00


==> implementation.tex <==
\Section{Implementation}
\label{sec:imp}
AdaCache extends Samsung PoseidonOS~\cite{inspur} to offer cache services for cloud block storage. It is implemented as a virtual block device (bdev) module under the SPDK framework. By using a virtual bdev module, AdaCache can be easily integrated with a wide range of cloud block storage bdevs, making it compatible with existing storage systems. AdaCache redirects I/Os between PoseidonOS and the cloud block storage based on whether there is a cache hit or miss, without requiring knowledge of the I/O protocol details of the underlying bdevs.

The AdaCache instance is initialized with a number of source-to-cache address mappings which equals to the number of available cache line sizes. The mappings are created using GLib's hash table data structure~\cite{}. During initialization, the AdaCache bdev obtains the cache bdev from PoseidonOS and core bdev from the cloud block storage to create the AdaCache bdev instance. The newly created AdaCache bdev is then made available to the cache client using SPDK's NVMeoF target~\cite{}.

AdaCache provides support for both write back and write through cache modes. When a read request is made, the I/O handling procedures are identical for both cache modes: data blocks are retrieved from the cloud block storage and placed into cache devices upon a cache miss, and served directly from the cache devices upon a cache hit.
% When a write request is made in write back cache mode, data blocks are written directly to the cache devices, regardless of whether there is a cache hit or miss except for compulsory misses. Dirty data blocks are written back to the cloud block storage either when they are evicted from the cache or during a periodic write-back process.
% In write through cache mode, data blocks are made persistent to the cloud block storage regardless of cache hit or miss when a write request is made.
% We use the hash table data structure of GLib~\cite{glib} to serve as the source-to-cache address mapping index. 


==> msr_replay_wss10.tex <==
rd_avg_lat_us	prn_1.csv	proj_1.csv	proj_2.csv	src1_0.csv	src1_1.csv	usr_1.csv	usr_2.csv
32k	270.60	232.82	214.11	302.34	221.91	241.34	242.76
64k	307.43	274.13	263.38	337.39	270.20	276.62	284.93
128k	373.40	341.58	329.63	387.97	331.86	336.40	351.71
256k	413.51	375.29	364.29	404.64	358.66	368.56	386.18
32k-256k	253.51	218.93	202.33	317.63	213.04	223.35	228.09
							
wr_avg_lat_us	prn_1.csv	proj_1.csv	proj_2.csv	src1_0.csv	src1_1.csv	usr_1.csv	usr_2.csv
32k	112.23	272.56	227.33	240.26	154.35	279.29	218.29
64k	134.22	257.97	205.93	244.30	156.37	262.16	214.21
128k	155.14	243.34	209.12	257.16	143.91	252.46	215.63
256k	186.28	245.12	211.47	267.90	166.03	261.89	221.50
32k-256k	112.97	248.32	211.89	240.49	152.15	266.44	202.76

process_each_req_lat_us	prn_1.csv	proj_1.csv	proj_2.csv	src1_0.csv	src1_1.csv	usr_1.csv	usr_2.csv
32k	5.89	13.90	14.13	10.34	8.72	14.60	12.95
64k	3.74	8.57	8.33	6.06	5.07	8.79	7.68
128k	2.36	5.21	5.85	3.61	3.09	5.21	5.15
256k	1.84	3.37	2.76	1.89	1.62	3.39	2.66
32k-256k	3.32	10.59	10.97	9.75	7.55	10.50	10.17

32k-256k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
21.00	7365331.00	101204806144.00	5064991.00	163046529024.00	2482752.00	141125976064.00	417095.00	16084041728.00	417095.00	16084041728.00	7563766.00	5210356.00	2436233.00	2306976.00	223316.00
60.00	9582079.00	198225741312.00	8497329.00	415310983168.00	6115412.00	381362667520.00	2868392.00	124282929152.00	2868392.00	124282929152.00	7444461.00	3288883.00	2555538.00	595961.00	535818.00
31.00	9129661.00	119352312832.00	7473401.00	400426053120.00	6423911.00	392242298880.00	220284.00	8319631360.00	220284.00	8319631360.00	9073731.00	2789685.00	926268.00	786406.00	2313730.00
32.00	9626731.00	133425643008.00	8100874.00	486085216256.00	7490401.00	478119624704.00	22832.00	848166912.00	22832.00	848166912.00	9492981.00	2148209.00	507018.00	361584.00	3382402.00
61.00	10286732.00	177545729536.00	5888076.00	254482637824.00	5365287.00	248764727296.00	135410.00	4587454464.00	135410.00	4587454464.00	9552627.00	4212500.00	447372.00	423947.00	3759526.00
101.00	13726514.00	288429113856.00	6058979.00	355424818176.00	5565765.00	351906562048.00	83215.00	2889318400.00	83215.00	2889318400.00	9549458.00	4028385.00	450541.00	406446.00	5422832.00
102.00	8559752.00	133368705024.00	8728089.00	448639784960.00	6769348.00	431226748928.00	137267.00	5459476480.00	137267.00	5459476480.00	8283424.00	1670060.00	1716575.00	1561116.00	6381515.00
															
32k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
21.00	7925969.00	102564561408.00	5123944.00	163395968512.00	2501529.00	141525090304.00	518667.00	16995680256.00	518667.00	16995680256.00	7563766.00	5192831.00	2436233.00	2305652.00	265152.00
60.00	10575410.00	198112556032.00	8538669.00	415826122752.00	6123030.00	381702668288.00	3793753.00	124313698304.00	3793753.00	124313698304.00	7444461.00	3275724.00	2555538.00	601259.00	662525.00
31.00	9279709.00	119282018304.00	7501500.00	400451488768.00	6424390.00	392267857920.00	252007.00	8257765376.00	252007.00	8257765376.00	9073731.00	2789257.00	926268.00	786356.00	2951384.00
32.00	9844730.00	133416737792.00	8156563.00	486096092672.00	7490631.00	478130634752.00	25679.00	841449472.00	25679.00	841449472.00	9492981.00	2147988.00	507018.00	361575.00	4295366.00
61.00	10875861.00	177556862464.00	5834799.00	254014386176.00	5296581.00	248310267904.00	140259.00	4596006912.00	140259.00	4596006912.00	9552627.00	4279501.00	447372.00	423934.00	4689717.00
101.00	15366385.00	288378107904.00	6084950.00	355670820864.00	5570221.00	352158154752.00	89293.00	2925953024.00	89293.00	2925953024.00	9549458.00	4024823.00	450541.00	405550.00	6848180.00
102.00	8746181.00	134000736256.00	8869033.00	448236004352.00	6764319.00	430831403008.00	167578.00	5491195904.00	167578.00	5491195904.00	8283424.00	1676096.00	1716575.00	1560102.00	8091509.00
															
64k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
21.00	7259971.00	124462287360.00	4723761.00	203061193216.00	2192438.00	179786547200.00	345053.00	22613393408.00	345053.00	22613393408.00	7563766.00	5459561.00	2436233.00	2348001.00	132575.00
60.00	8913948.00	257477657088.00	7038131.00	447541950464.00	4578837.00	383062310912.00	1917947.00	125694574592.00	1917947.00	125694574592.00	7444461.00	4412883.00	2555538.00	1008279.00	331261.00
31.00	8976329.00	211358024192.00	5699541.00	409503048192.00	4706524.00	399452930048.00	149722.00	9812180992.00	149722.00	9812180992.00	9073731.00	4475537.00	926268.00	817938.00	1475690.00
32.00	9529030.00	250825481216.00	6238995.00	491749221888.00	5654122.00	481595359232.00	16915.00	1108541440.00	16915.00	1108541440.00	9492981.00	3944636.00	507018.00	401241.00	2147680.00
61.00	10299391.00	238546530816.00	3831502.00	256471299584.00	3340219.00	250588561408.00	104625.00	6856704000.00	104625.00	6856704000.00	9552627.00	6230722.00	447372.00	429058.00	2344855.00
101.00	12314245.00	373077500928.00	4587035.00	360060400128.00	4109026.00	356075634688.00	62574.00	4100849664.00	62574.00	4100849664.00	9549458.00	5475823.00	450541.00	415151.00	3424086.00
102.00	8356907.00	235876402688.00	6934640.00	457907385344.00	5037815.00	438359228416.00	102062.00	6688735232.00	102062.00	6688735232.00	8283424.00	3357052.00	1716575.00	1605174.00	4045750.00
															
128k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
21.00	6912874.00	150652253696.00	4264689.00	284749408256.00	1788031.00	260337958912.00	268238.00	35158491136.00	268238.00	35158491136.00	7563766.00	5834322.00	2436233.00	2377646.00	66287.00
60.00	8155428.00	312737001472.00	5037446.00	477454292480.00	2528696.00	385444741120.00	975181.00	127818924032.00	975181.00	127818924032.00	7444461.00	5750574.00	2555538.00	1720729.00	165629.00
31.00	8883239.00	281277642752.00	3718459.00	422576984576.00	2760051.00	410974027776.00	93503.00	12255625216.00	93503.00	12255625216.00	9073731.00	6375387.00	926268.00	864561.00	737843.00
32.00	9415653.00	341451707392.00	3784529.00	499631540224.00	3239623.00	487846969344.00	30062.00	3940286464.00	30062.00	3940286464.00	9492981.00	6314655.00	507018.00	445721.00	1073837.00
61.00	9928290.00	282304190464.00	2318259.00	260198468096.00	1851148.00	254175608832.00	78120.00	10239344640.00	78120.00	10239344640.00	9552627.00	7714096.00	447372.00	434755.00	1172424.00
101.00	10792320.00	439755597312.00	2858268.00	366895276544.00	2396780.00	362543841280.00	45184.00	5922357248.00	45184.00	5922357248.00	9549458.00	7174243.00	450541.00	428976.00	1712039.00
102.00	8223868.00	315757840896.00	4759024.00	468514381824.00	2952915.00	447343099904.00	66999.00	8781692928.00	66999.00	8781692928.00	8283424.00	5398137.00	1716575.00	1648971.00	2022870.00
															
256k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
21.00	6868073.00	193618158592.00	3857665.00	415383293952.00	1416778.00	390073679872.00	241435.00	63290736640.00	241435.00	63290736640.00	7563766.00	6194900.00	2436233.00	2388321.00	33143.00
60.00	7780514.00	350708778496.00	3930923.00	496749373952.00	1395250.00	388051501056.00	499528.00	130948268032.00	499528.00	130948268032.00	7444461.00	6487976.00	2555538.00	2116773.00	82813.00
31.00	8848928.00	333134811648.00	2495138.00	442631171584.00	1554012.00	430047494144.00	63625.00	16678912000.00	63625.00	16678912000.00	9073731.00	7552858.00	926268.00	893129.00	368919.00
32.00	9342860.00	402437517824.00	2321061.00	512004908032.00	1796257.00	499097010176.00	18419.00	4828430336.00	18419.00	4828430336.00	9492981.00	7730247.00	507018.00	473495.00	536915.00
61.00	9734731.00	310798656000.00	1437249.00	266182321664.00	981985.00	260067295232.00	56767.00	14881128448.00	56767.00	14881128448.00	9552627.00	8579306.00	447372.00	438708.00	586208.00
101.00	10023012.00	488285187072.00	1800856.00	377676165632.00	1347351.00	373102215168.00	33683.00	8829796352.00	33683.00	8829796352.00	9549458.00	8215259.00	450541.00	437389.00	856015.00
102.00	8157216.00	373216909312.00	3433155.00	489233233408.00	1675263.00	466810306560.00	47211.00	12376080384.00	47211.00	12376080384.00	8283424.00	6646845.00	1716575.00	1677897.00	1011430.00


==> simulation_results.tex <==
alibaba	avg_read_hit_%	avg_write_hit_%	cache_read_TB	cache_write_TB	core_read_TB	core_write_TB	avg_blk_sz	stdev_blk_sz	min_blksz	max_blksz
var	89.40	89.70	374.71	528.10	320.11	262.00	42.93	11.22	32.77	106.28
32K	88.91	89.42	376.81	530.60	324.65	264.96	32.00	32.00	32.00	32.00
64K	90.65	91.16	383.74	548.43	331.23	268.20	64.00	64.00	64.00	64.00
128K	92.13	93.44	394.67	581.99	343.15	273.48	128.00	128.00	128.00	128.00
256K	94.46	94.91	414.44	621.28	362.36	282.65	256.00	256.00	256.00	256.00

msr	avg_read_hit_%	avg_write_hit_%	cache_read_TB	cache_write_TB	core_read_TB	core_write_TB	avg_blk_sz	stdev_blk_sz	min_blksz	max_blksz
var	48.27	50.49	4.27	5.99	5.60	1.02	41.35	1.68	37.94	42.83
32K	48.40	50.54	4.27	5.98	5.59	1.02	32.00	32.00	32.00	32.00
64K	62.65	61.51	5.38	6.32	5.70	1.05	64.00	64.00	64.00	64.00
128K	78.23	78.90	6.28	6.69	5.87	1.11	128.00	128.00	128.00	128.00
256K	87.63	88.76	6.94	7.11	6.16	1.20	256.00	256.00	256.00	256.00

systor	avg_read_hit_%	avg_write_hit_%	cache_read_TB	cache_write_TB	core_read_TB	core_write_TB	avg_blk_sz	stdev_blk_sz	min_blksz	max_blksz
var	69.67	89.84	59.90	76.78	65.44	12.23	40.41	0.99	38.90	42.14
32K	69.09	89.64	59.85	75.81	64.43	12.09	32.00	32.00	32.00	32.00
64K	74.82	90.97	66.79	88.32	75.91	13.40	64.00	64.00	64.00	64.00
128K	79.71	92.02	77.16	109.45	95.14	15.65	128.00	128.00	128.00	128.00
256K	85.32	94.99	88.91	146.56	130.38	20.20	256.00	256.00	256.00	256.00

alibaba	le4k	le8k	le16k	le32k	le64k	le128k	le256k	gt256k
sum	12843287852.00	1509332494.00	1861212779.00	1249103600.00	1103469093.00	383834040.00	502691073.00	780042420.00
acc	12843287852.00	14352620346.00	16213833125.00	17462936725.00	18566405818.00	18950239858.00	19452930931.00	20232973351.00
cdf	63.48	70.94	80.14	86.31	91.76	93.66	96.14	100.00

msr	le4k	le8k	le16k	le32k	le64k	le128k	le256k	gt256k
sum	54749012.00	5682421.00	4218863.00	28010238.00	110472391.00	2141.00	2064.00	18366.00
accu	54749012.00	60431433.00	64650296.00	92660534.00	203132925.00	203135066.00	203137130.00	203155496.00
cdf	26.95	29.75	31.82	45.61	99.99	99.99	99.99	100.00

systor	le4k	le8k	le16k	le32k	le64k	le128k	le256k	gt256k
sum	2205351706.00	333638406.00	328371164.00	702165242.00	222518415.00	204456794.00	299454294.00	1678985.00
accu	2205351706.00	2538990112.00	2867361276.00	3569526518.00	3792044933.00	3996501727.00	4295956021.00	4297635006.00
cdf	51.32	59.08	66.72	83.06	88.24	92.99	99.96	100.00

disk_id	avg_req	avg_cl_sz
vd2	23.30	39.47
vd10	84.24	64.60
vd49	31.14	41.79
vd124	14.68	36.33
bd740	10.68	35.52
		
disk_id	avg_req	avg_cl_sz
prn_1	30.66	41.19
proj_1	45.96	45.34
proj_2	56.72	47.02
src1_0	52.27	45.64
src1_1	32.71	36.30
usr_1	53.57	46.58
usr_2	54.85	46.74
		
disk_id	avg_req	avg_cl_sz
LUN0	25.52	40.54
LUN1	27.74	41.16
LUN2	19.13	37.46
LUN3	22.65	39.83
LUN4	24.63	40.28
LUN6	20.44	39.15


==> systor_replay_wss10.tex <==
rd_avg_lat_us	lun0.csv	lun1.csv	lun2.csv	lun3.csv	lun4.csv	lun6.csv
32k	193.79	194.53	184.62	196.14	184.03	193.76
64k	196.20	189.94	183.77	190.27	183.60	191.19
128k	227.72	221.59	207.64	219.43	210.86	224.20
256k	263.64	252.71	239.51	257.67	243.46	254.42
32k-256k	194.96	190.01	181.87	193.16	184.45	191.65
						
wr_avg_lat_us	lun0.csv	lun1.csv	lun2.csv	lun3.csv	lun4.csv	lun6.csv
32k	298.86	316.68	305.12	327.51	358.42	316.97
64k	299.81	326.37	314.77	336.35	362.53	322.53
128k	304.11	329.44	312.20	337.91	360.65	330.49
256k	313.52	336.88	322.94	347.52	363.91	342.28
32k-256k	291.09	322.76	311.65	330.03	359.89	322.49

process_each_req_lat_us	lun0.csv	lun1.csv	lun2.csv	lun3.csv	lun4.csv	lun6.csv
32k	7.25	8.49	8.39	8.25	9.11	8.58
64k	5.57	6.54	6.37	6.42	6.88	6.61
128k	4.41	4.94	4.72	5.03	5.16	5.06
256k	3.56	3.90	3.77	4.06	4.02	3.96
32k-256k	7.68	9.13	8.47	8.76	9.60	9.04

32k-256k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
lun0.csv	6043398.00	93455150080.00	7053797.00	199906025984.00	2606842.00	162749775872.00	127462.00	5987139584.00	127462.00	5987139584.00	5870793.00	3640663.00	4129206.00	3757753.00	3108282.00
lun1.csv	6613229.00	109353157120.00	6787304.00	229174766592.00	2991297.00	198093537280.00	133054.00	6700531712.00	133054.00	6700531712.00	6452838.00	3825372.00	3547161.00	3189205.00	6480826.00
lun2.csv	7426342.00	97178130944.00	5848069.00	220683613696.00	3315245.00	200791228416.00	264631.00	12571377664.00	264631.00	12571377664.00	7548899.00	4536429.00	2451100.00	2153912.00	9621870.00
lun3.csv	6551860.00	102686046208.00	6544987.00	213351417344.00	2970419.00	187500593152.00	137193.00	6773211136.00	137193.00	6773211136.00	6589869.00	3955696.00	3410130.00	3080926.00	13212236.00
lun4.csv	7608510.00	109608808960.00	5879076.00	242485761024.00	3359043.00	221674176512.00	158756.00	7985037312.00	158756.00	7985037312.00	7622718.00	4523106.00	2377281.00	2122849.00	16851077.00
lun6.csv	6555357.00	100541142016.00	6896664.00	242398610944.00	3231325.00	206178975744.00	190596.00	9440362496.00	190596.00	9440362496.00	6640555.00	3794399.00	3359444.00	2981061.00	20105486.00
															
32k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
lun0.csv	5806785.00	93703680512.00	6952828.00	199800669696.00	2607097.00	162653503488.00	184861.00	6057525248.00	184861.00	6057525248.00	5870793.00	3640605.00	4129206.00	3757391.00	3973816.00
lun1.csv	6378811.00	109106428928.00	6734441.00	229003168256.00	2989072.00	198001229824.00	191142.00	6263341056.00	191142.00	6263341056.00	6452838.00	3829912.00	3547161.00	3186780.00	8263268.00
lun2.csv	7323049.00	97205540352.00	5815074.00	220813752320.00	3317854.00	200925806592.00	386320.00	12658933760.00	386320.00	12658933760.00	7548899.00	4534080.00	2451100.00	2153728.00	12356220.00
lun3.csv	6284316.00	102180152832.00	6497484.00	213482149376.00	2973567.00	187640512512.00	192781.00	6317047808.00	192781.00	6317047808.00	6589869.00	3953019.00	3410130.00	3080499.00	17022259.00
lun4.csv	7388810.00	107814052352.00	5849431.00	243321524224.00	3376244.00	222545543168.00	200309.00	6563725312.00	200309.00	6563725312.00	7622718.00	4506740.00	2377281.00	2121885.00	21725657.00
lun6.csv	6378281.00	100668852736.00	6794471.00	242817355776.00	3240633.00	206638710784.00	296671.00	9721315328.00	296671.00	9721315328.00	6640555.00	3786769.00	3359444.00	2979356.00	25884084.00
															
64k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
lun0.csv	5729082.00	111853941760.00	6277414.00	223831982080.00	2005711.00	183212244992.00	121872.00	7987003392.00	121872.00	7987003392.00	5870793.00	4169927.00	4129206.00	3825042.00	1986907.00
lun1.csv	6267766.00	131805416960.00	6001004.00	255491655680.00	2350475.00	220940664832.00	126773.00	8308195328.00	126773.00	8308195328.00	6452838.00	4400257.00	3547161.00	3250011.00	4131632.00
lun2.csv	7225304.00	119683041792.00	4978699.00	247496909312.00	2510312.00	224607338496.00	231244.00	15154806784.00	231244.00	15154806784.00	7548899.00	5297191.00	2451100.00	2193098.00	6178107.00
lun3.csv	6258527.00	123912962048.00	5790681.00	240971919872.00	2335138.00	212164149248.00	128013.00	8389459968.00	128013.00	8389459968.00	6589869.00	4530141.00	3410130.00	3135803.00	8511126.00
lun4.csv	7370889.00	136015663616.00	5030314.00	267440139264.00	2608432.00	244090535936.00	145251.00	9519169536.00	145251.00	9519169536.00	7622718.00	5231367.00	2377281.00	2160912.00	10862824.00
lun6.csv	6285542.00	123203729408.00	6034643.00	272755354112.00	2550289.00	232899215360.00	165105.00	10820321280.00	165105.00	10820321280.00	6640555.00	4410710.00	3359444.00	3039935.00	12942037.00
															
128k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
lun0.csv	5681069.00	136822038016.00	5704759.00	262877332992.00	1510688.00	216577605632.00	96472.00	12644777984.00	96472.00	12644777984.00	5870793.00	4612296.00	4129206.00	3877015.00	993453.00
lun1.csv	6233363.00	166642387968.00	5384407.00	298711568384.00	1797286.00	258400321536.00	122846.00	16101670912.00	122846.00	16101670912.00	6452838.00	4906661.00	3547161.00	3296052.00	2065815.00
lun2.csv	7202428.00	152892420096.00	4348322.00	293080677376.00	1903320.00	265007792128.00	168108.00	22034251776.00	168108.00	22034251776.00	7548899.00	5874964.00	2451100.00	2221715.00	3089052.00
lun3.csv	6226449.00	153854172160.00	5222313.00	290927354880.00	1818081.00	257292763136.00	100312.00	13148094464.00	100312.00	13148094464.00	6589869.00	5007465.00	3410130.00	3174453.00	4255561.00
lun4.csv	7319117.00	173093484544.00	4377816.00	308321678848.00	1989397.00	280946016256.00	97086.00	12725256192.00	97086.00	12725256192.00	7622718.00	5818956.00	2377281.00	2191646.00	5431409.00
lun6.csv	6243921.00	156376194048.00	5401486.00	325158929408.00	1981335.00	279019913216.00	124295.00	16291594240.00	124295.00	16291594240.00	6640555.00	4931726.00	3359444.00	3086938.00	6471015.00
															
256k															
disk_id	cache_read_cnt	cache_read_bytes	cache_write_cnt	cache_write_bytes	core_read_cnt	core_read_bytes	core_write_cnt	core_write_bytes	eviction_cnt	eviction_bytes	read_cnt	read_hit	write_cnt	write_hit	total_cls
lun0.csv	5654330.00	166814605824.00	5150487.00	329194553856.00	1006915.00	277814444032.00	99364.00	26047676416.00	99364.00	26047676416.00	5870793.00	5021064.00	4129206.00	3972020.00	496726.00
lun1.csv	6204654.00	198843940352.00	4713593.00	367977709568.00	1167084.00	322414313472.00	94653.00	24812716032.00	94653.00	24812716032.00	6452838.00	5439774.00	3547161.00	3393141.00	1032906.00
lun2.csv	7181742.00	183624653312.00	3668091.00	369997989376.00	1240179.00	336726065152.00	116155.00	30449336320.00	116155.00	30449336320.00	7548899.00	6450425.00	2451100.00	2309395.00	1544524.00
lun3.csv	6221487.00	183115241472.00	4604484.00	372895215104.00	1222914.00	334895775744.00	81165.00	21276917760.00	81165.00	21276917760.00	6589869.00	5518656.00	3410130.00	3258429.00	2127778.00
lun4.csv	7304811.00	208125771776.00	3616131.00	373933483520.00	1250192.00	342686171136.00	70541.00	18491899904.00	70541.00	18491899904.00	7622718.00	6487153.00	2377281.00	2262654.00	2715701.00
lun6.csv	6237178.00	190332871168.00	4682848.00	411143540224.00	1315101.00	359297974272.00	101695.00	26658734080.00	101695.00	26658734080.00	6640555.00	5498987.00	3359444.00	3185911.00	3235503.00

